Comparing representations of biological data learned with different AI paradigms, augmenting and cropping strategies

Recent advances in computer vision and robotics enabled automated large-scale biological image analysis. Various machine learning approaches have been successfully applied to phenotypic profiling. However, it remains unclear how they compare in terms of biological feature extraction. In this study, we propose a simple CNN architecture and implement 4 different representation learning approaches. We train 16 deep learning setups on the 770k cancer cell images dataset under identical conditions, using different augmenting and cropping strategies. We compare the learned representations by evaluating multiple metrics for each of three downstream tasks: i) distance-based similarity analysis of known drugs, ii) classification of drugs versus controls, iii) clustering within cell lines. We also compare training times and memory usage. Among all tested setups, multi-crops and random augmentations generally improved performance across tasks, as expected. Strikingly, self-supervised (implicit contrastive learning) models showed competitive performance being up to 11 times faster to train. Self-supervised regularized learning required the most of memory and computation to deliver arguably the most informative features. We observe that no single combination of augmenting and cropping strategies consistently results in top performance across tasks and recommend prospective research directions.

==> hacks/many-authors-hack.tex <==
%\begin{comment}
\makeatletter
% hack the footer of the title page as it doesn't seem to automatically use the et al. version when spanning acros multiple pages
\renewcommand*{\@titlefoot}{\scriptsize\copyright\space\@jmlryear
    \ifanonsubmission
    \space Author(s) names withheld.\hfill
    \else
    \space \@firstauthor\space \emph{et al}.\hfill
    \@reprint
    \fi
  }
\makeatother
%\end{comment}

% \begin{comment}
\makeatletter
% remove the vbox in @jmlrmaketitle which prevents the text to be split across several pages
\renewcommand{\@jmlrmaketitle}{
  % specify the page style in case it spans over several pages. Not sure why this is needed
  \thispagestyle{jmlrtps}%
  % define a new label for the first page as otherwise it starts from 2 in the header
  \label{jmlrstartnew}%
  % hack the spacing to mimick what happens with a vbox
  \null\vspace{-\parindent}\vspace{-2pt}{
  \hsize\textwidth
  \linewidth\hsize
 \jmlrpretitle
  {%
    \def\titletag##1{##1}%
    \@title
  }%
 \jmlrposttitle
 \jmlrpreauthor \@author \jmlrpostauthor
}
% hack the spacing to mimick what happens with a vbox
\vspace{2pt}
}
\makeatother
%\end{comment}

%\begin{comment}
\makeatletter
% hack the footer to use the new counter
\renewcommand*\@jmlrpages{\pageref{jmlrstartnew}--\pageref{jmlrend}}
\makeatother
%\end{comment}
